A Near-Linear Time Approximation Algorithm for Beyond-Worst-Case Graph Clustering

We consider the semi-random graph model of [Makarychev, Makarychev and Vijayaraghavan, STOC'12], where, given a random bipartite graph with $\alpha$ edges and an unknown bipartition $(A, B)$ of the vertex set, an adversary can add arbitrary edges inside each community and remove arbitrary edges from the cut $(A, B)$ (i.e. all adversarial changes are \textit{monotone} with respect to the bipartition). For this model, a polynomial time algorithm is known to approximate the Balanced Cut problem up to value $O(\alpha)$ [MMV'12] as long as the cut $(A, B)$ has size $\Omega(\alpha)$. However, it consists of slow subroutines requiring optimal solutions for logarithmically many semidefinite programs. We study the fine-grained complexity of the problem and present the first near-linear time algorithm that achieves similar performances to that of [MMV'12]. Our algorithm runs in time $O(|V(G)|^{1+o(1)} + |E(G)|^{1+o(1)})$ and finds a balanced cut of value $O(\alpha)$. Our approach appears easily extendible to related problem, such as Sparsest Cut, and also yields an near-linear time $O(1)$-approximation to Dagupta's objective function for hierarchical clustering [Dasgupta, STOC'16] for the semi-random hierarchical stochastic block model inputs of [Cohen-Addad, Kanade, Mallmann-Trenn, Mathieu, JACM'19].

==> content/lower_bound.tex <==
\section{Lower Bound}

In this section, we show that the dependency in $\sqrt{\log n}$ is tight. Let us focus on the bisection problem.
\Vnote{In fact, the dependency is $O(\sqrt{\log n} \log \log n)$, right? I think this is tight for non-uniform sparsest cut, so maybe the proof
  has to be adapted to this to get an exactly tight result}.


There are two types of lower bounds: The best possible polytime approximation under the UGC, and the integrality gap of the SDP-based state-of-the-art
algorithm for the problem.

Let $\mathcal I$ be a family of hard instance for the integrality gap of the SDP-based state-of-the-art algorithm for the problem. For this, the adversary
takes an instance with an integrality gap of $\Theta(\sqrt{\log n})$ on $n/2$ vertices \Vnote{Add ref}.
Let $q$ be the number of edges in the optimum integral cut of this instance and let $L,R$ be the two sides of the cut. 
Now, the adversary builds the following graph in our model. First it generates the planted cut between sides $A,B$
so that the expected number of edges in the planted cut
is $\Theta(q)$. Then, on side $A$ of the model, it plants (arbitrarily) the above instance and proceeds identically on $B$.
Let $L_A,R_A$ and $L_B,R_B$
the corresponding four sets hence defined. Next, the adversary removes all edges $(u,v)$ such that either $u \in L_A$ and $v \in R_B$ or $u \in R_A$ and
$u \in L_B$. We obtain the following properties on the resulting graph:
\begin{enumerate}
\item The planted cut $(A,B)$ contains $\Theta(q)$ after removal of the edges (only 1/2 of the edges have been removed).
\item The cut $(L_A \cup L_B, R_A \cup R_B)$ is of value $2q$.
\item The SDP solution which consists in taking the SDP solution for $L,R$ and providing the same embedding for the two copies of the same vertex has
  cost at most twice its cost for $L,R$. 
\end{enumerate}
Since the gap is $\Theta(\sqrt{\log n})$ for the graph $L,R$, the optimal SDP solution has cost at most $O(q/ \sqrt{\log n})$ while any other cut
has cost at least $q$.






==> content/oracle.tex <==




We divide the proof of \cref{theorem:oracle-main} into different lemmas. The first two steps are just rephrasing of results in \cite{DBLP:conf-stoc-AroraK07,DBLP:conf-focs-Sherman09}. As in previous sections, we denote the optimal objective value of \cref{eq:extended-balanced-cut-primal-sdp} by $\alpha$.

\begin{lemma}[\cite{DBLP:conf-stoc-AroraK07}]
	%Consider the settings of \cref{theorem:oracle-main}.
	Consider the parameter settings of \cref{theorem:oracle-main}.
	There exists a  $\tilde{O}(\alpha/n)$-bounded, $O(\log n)^{100}$-robust, $\Theta(1)$-separation oracle that, given a candidate solution to \cref{eq:extended-balanced-cut-primal-sdp} with input graph $G$ on $n$ vertices, outputs \textbf{no} if one of the following conditions is violated:
	\begin{enumerate}
		\item[(flatness):] $W:=\Set{i\in [n]\suchthat \Snorm{v_i}>2} \subseteq [n]$  satisfies $\Card{W}< \frac{n}{(\log n)^{100}}$.
		\item[(balance):] $S:= [n]\setminus W$ satisfies $\sum_{i,j \in S} \Snorm{v_i-v_j}\geq 2an$.  
	\end{enumerate}
	Moreover, if the candidate solution is given in the form of $v_1,\ldots, v_n\in \R^{O(\polylog n)}$, the oracle runs in time $\tilde{O}(\card{V(G)}+\card{E(G)})$.
	Finally, in the \textbf{no} case  the resulting feedback matrix has $O(m+n)$ non-zero entries.
\end{lemma}

We omit the proof of \cref{lemma:basic-oracle} as it can be found in \cite{DBLP:conf-stoc-AroraK07}.
If both the flatness and the balance condition are satisfied, then we apply the following \oracle,   due to \cite{DBLP:conf-stoc-AroraK07, DBLP:conf-focs-Sherman09}.

\begin{lemma}[\cite{DBLP:conf-stoc-AroraK07}]
	Consider the parameter settings of \cref{theorem:oracle-main}.
	There exists a  $\tilde{O}(\alpha/\ell\cdot n)$-bounded, $O(\log n)^{100}$-robust, $\Theta(1)$-separation oracle that, given a candidate solution to \cref{eq:extended-balanced-cut-primal-sdp} with input graph $G$ on $n$ vertices and optimal cut of  value at most $\alpha$, % with probability $1-(\log n)^{-100}$ over random bits, 
	outputs \textbf{yes} only if it finds a $(a/10)$-balanced cut of value $O(\alpha)$, or an $(a/10)$-balanced partition $(P, P')$ of $V(G)$ satisfying
	\begin{align*}
		\sum_{i \in P\,, j \in P'\,, \ij \in E(G)} \Snorm{v_i-v_j}&\leq O(\alpha)\\
		\Card{E(P, P')}&\leq O(\alpha\cdot \rho)\cdot \sqrt{\log n}\,.
	\end{align*}
	Furthermore, the oracle outputs \textbf{no} with probability at least $1-O(\log n)^{-100}$ over random bits if
	\begin{align*}
	\Card{\Set{\ij \in V(G)\suchthat \Snorm{v_i-v_j}\geq \delta} }\leq O\Paren{\frac{\alpha}{\delta}}\,.
	\end{align*}

	Moreover, if the candidate solution is given in the form of $v_1,\ldots, v_n \in \R^{O(\polylog n)}$, the oracle runs in time $\tilde{O}\Paren{\Card{V(G)}^{1+O(1/\rho^2)}+\Card{E(G)}^{1+O(1/\rho^2)}}$. Finally, in the \textbf{no} case  the resulting feedback matrix has $O(m+n)$ non-zero entries.
\end{lemma}

The proof of \cref{lemma:flow-oracle} can be found in \cite{DBLP:conf-focs-Sherman09}.%, we reproduce it in \cref{section:missing-proofs}. 
The improvement on the time complexity simply follows using \cref{theorem:max-flow-linear-time}.
The next result is the \textit{crucial} addition we need to the \oracle of \cite{DBLP:conf-stoc-AroraK07,DBLP:conf-focs-Sherman09}.  We prove it in \cref{section:bounded-oracle-heavy-vertices}.

\begin{lemma}
	Consider the parameter settings of \cref{theorem:oracle-main}.
	
	Let $G$ be a graph on $\ell \cdot n$ vertices with optimal cut of value at most $\alpha$ that is geometrically expanding up to scale $(\delta, n)$. 
	
	There exists a $\tilde{O}(\alpha/\ell\cdot n)$-bounded, $O(\log n)^{100}$-robust, $\Theta(1)$-separation oracle that, given a candidate solution to \cref{eq:extended-balanced-cut-primal-sdp} with input graph $G$, either outputs \textbf{no}, or outputs a set of edges $E^*\subseteq E(G)$ of cardinality $O(\alpha/\delta)$ and partition $(P_1, P_2, V')$ of $V(G)$ such that
	\begin{enumerate}
		\item[(1)] %$\Card{E(P_1, P_2, V')\cap \Set{\ij \in E(G)\suchthat \Snorm{v_i-v_j}\leq \delta}}\leq O\Paren{ \frac{\alpha}{\delta}\Paren{1+\frac{\ell}{\delta}}}\,.$
		 $\Card{E(P_1, P_2, V')\setminus E^*}\leq O\Paren{ \frac{\alpha}{\rho\delta}\Paren{1+\frac{\ell}{\rho\delta}}}\,.$
		\item[(2)]  $\Abs{\Card{P_1} - \Card{P_2}} \leq an/2$ or $\Card{V'}\geq an/10\,.$
		\item[(3)]%the optimal $a$-balanced cut on $V'$ has value at most $10\alpha \delta^2$. 
						$\forall \ij \in E(G)\setminus E^*$ with $i,j \in V'$ it holds $\Snorm{v_i-v_j}\leq \delta\,.$
		\item[(4)] $H_{\delta, n}(X, V')=\emptyset\,.$ 
	\end{enumerate}

	Moreover, if the candidate solution is given in the form of $v_1,\ldots, v_n \in \R^{O(\polylog n)}$, the oracle runs in time $\tilde{O}\Paren{\rho\cdot \Card{V(G)}^{1+O(1/\rho^2)}+\rho\cdot \Card{E(G)}^{1+O(1/\rho^2)}}$.
	Finally, in the \textbf{no} case  the resulting feedback matrix has $O(m+n)$ non-zero entries.
\end{lemma}


Together, these Lemmata immediately imply \cref{theorem:oracle-main}.








































==> content/practical.tex <==
\begin{remark}[On practical implementations of the algorithm]\label{remark:practical-implementations}
	The following precautions should be taken into account upon implementing the algorithm.
	First, replace the subroutine of \cite{DBLP:conf-focs-Sherman09} with a simple maximum-flow computation as in \cite{DBLP:conf-stoc-AroraK07}. Note that this different subroutine provides worse approximation guarantees by a  $O(\sqrt{\log n})$ factor. Nevertheless, the algorithms still provides the same error guarantees if one increases proportionally the number of iterations of the main procedure. Second, replace the maximum flow algorithm of \cref{theorem:max-flow-linear-time} with a more practical --even if asymptotically slower-- maximum flow algorithm. We remark that with these modifications, the algorithm amounts to a sequence of basic computations such as: matrix-vector multiplications, hash-functions and max-flow computations.
\end{remark}

\begin{remark}[On potential practical implementations]
	It is important to remark that we believe the hidden constant behind the algorithm of \cref{theorem:main} to be small. In particular, we do not try to optimize the constants appearing in our analysis and therefore they should not be seen as an inherent barrier to practical implementations.  We explain few precautions needed for potential practical implementations after introducing \cref{algorithm:balanced-cut}.  
\end{remark}
